Easy to Decide, Hard to Agree: Reducing Disagreements Between Saliency Methods

A popular approach to unveiling the black box of neural NLP models is to leverage saliency methods, which assign scalar importance scores to each input component. A common practice for evaluating whether an interpretability method is faithful has been to use evaluation-by-agreement -- if multiple methods agree on an explanation, its credibility increases. However, recent work has found that saliency methods exhibit weak rank correlations even when applied to the same model instance and advocated for the use of alternative diagnostic methods. In our work, we demonstrate that rank correlation is not a good fit for evaluating agreement and argue that Pearson-$r$ is a better-suited alternative. We further show that regularization techniques that increase faithfulness of attention explanations also increase agreement between saliency methods. By connecting our findings to instance categories based on training dynamics, we show that the agreement of saliency method explanations is very low for easy-to-learn instances. Finally, we connect the improvement in agreement across instance categories to local representation space statistics of instances, paving the way for work on analyzing which intrinsic model properties improve their predisposition to interpretability methods.

==> 6-regularizing-agreement.tex <==
\section{Improving Agreement Through Regularization}
\label{sec:regularizing-agreement}

Now that we know on which instance categories models tend to disagree on, our next goal is to attempt to fix these disagreements.
Most saliency methods are based on gradient information -- either directly using gradient information \cite{denil2014extraction,sundararajan2017axiomatic} or modifying the rules of backpropagation \cite{bach2015pixel,shrikumar2017learning}.
It is our hypothesis that because easy-to-classify instances, in particular, are correctly classified with high confidence from the first time the model encounters them, they receive small updates from backpropagation in subsequent epochs.
We believe this causes the local representation space around that concrete instance to possibly be sharp -- which is problematic for methods that leverage gradient-based information as each incorporates different notions of locality.
To alleviate these issues, we leverage two methods that have been shown to improve the faithfulness of attention-based explanations in conicity \cite{mohankumar2020towards} and tying \cite{tutek2020staying}.
\josip{maybe drop the first part?}
Our motivation is that although the cross entropy loss will still produce little signal to the model, the signal from the regularization term will be enough to sufficiently explore the local space, making it smoother and thus increasing agreement.

\todo{Popuniti tekst bulleta}
\begin{enumerate}
    \item Describe regularization methods
    \item Results: improved agreement (on average)
    \begin{itemize}
        \item In addition to graphs, also add improvement <on average> for each reg. method wrt. baseline
    \end{itemize}
    \item Results: improved agreement wrt. cartography
    \item Result analysis
\end{enumerate}


\begin{table}
\small
\caption{Top $F_1$ score across epochs \todo{caption}}
\label{tab:repr_dbert}
\begin{center}
\begin{tabular}{lrrrr}
\toprule
& & Non-reg & Conicity & Tying \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{dbert}}}
& SUBJ & $.93_{.01}$ & $.90_{.02}$ & $.93_{.00}$ \\
& SST & $.83_{.00}$ & $.83_{.01}$ & $.82_{.01}$ \\
& TREC & $.92_{.01}$ & $.92_{.01}$ & $.91_{.01}$ \\
& IMDB & $.86_{.01}$ & $.86_{.01}$ & $.88_{.00}$ \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{jwa}}}
& SUBJ & $.92_{.00}$ & $.90_{.00}$ & $.89_{.00}$ \\
& SST & $.78_{.04}$ & $.76_{.02}$ & $.78_{.02}$ \\
& TREC & $.89_{.02}$ & $.86_{.01}$ & $.89_{.01}$ \\
& IMDB & $.89_{.00}$ & $.88_{.00}$ & $.86_{.00}$ \\
\bottomrule
\end{tabular}
\end{center}
\end{table}
